Sneaking Up On The Criegee Intermediate From Below: Predicted Photoelectron Spectrum Of The CH_2OO^- Anion And W3-F12 Electron Affinity Of CH_2OO

High level ab initio calculations were undertaken on the CH$_2$OO anion and neutral species to predict the electron affinity and anion photoelectron spectrum. The electron affinity of CH$_2$OO, 0.567 eV, and barrier height for dissociation of CH$_2$OO$^-$ to O$^-$ and CH$_2$O, 16.5 kJ mol$^{-1}$, are obtained by means of the W3-F12 thermochemical protocol. Two major geometric differences between the anion and neutral, being the dihedral angle of the terminal hydrogen atoms with respect to C-O-O plane, and the O-O bond length, are reflected in the predicted spectrum as pronounced vibrational progressions.

==> metadata.tex <==
\hypersetup{
    pdfauthor={Marcus Kettner},
    pdftitle={Sneaking Up On The Criegee Intermediate From Below:},
    pdfsubject={Predicted Photoelectron Spectrum Of The CH_2OO^- Anion And W3-F12 Electron Affinity Of CH_2OO},
    pdfkeywords={Quantum Chemistry, Laser Chemistry, Physical Chemistry, Chemical Physics, Spectroscopy}
}

